Intervention Generalization: A View from Factor Graph Models

One of the goals of causal inference is to generalize from past experiments and observational data to novel conditions. While it is in principle possible to eventually learn a mapping from a novel experimental condition to an outcome of interest, provided a sufficient variety of experiments is available in the training data, coping with a large combinatorial space of possible interventions is hard. Under a typical sparse experimental design, this mapping is ill-posed without relying on heavy regularization or prior distributions. Such assumptions may or may not be reliable, and can be hard to defend or test. In this paper, we take a close look at how to warrant a leap from past experiments to novel conditions based on minimal assumptions about the factorization of the distribution of the manipulated system, communicated in the well-understood language of factor graph models. A postulated $\textit{interventional factor model}$ (IFM) may not always be informative, but it conveniently abstracts away a need for explicitly modeling unmeasured confounding and feedback mechanisms, leading to directly testable claims. Given an IFM and datasets from a collection of experimental regimes, we derive conditions for identifiability of the expected outcomes of new regimes never observed in these training data. We implement our framework using several efficient algorithms, and apply them on a range of semi-synthetic experiments.

==> 03_ifm_backup.tex <==
\section{Interventional Factor Model: Identification}
\label{sec:ifm_model}

We define our \emph{identification problem} as follows: given the population distribution functions $p(x; \sigma^1), p(x; \sigma^2), \dots, p(x; \sigma^t)$ for regimes $\Sigma_{train} := \{\sigma^1, \sigma^2, \dots, \sigma^t\}$, and knowledge of the factorization assumptions as given by Eq. (\ref{eq:ifm}), can we identify a given $p(x; \sigma^\star)$ corresponding to some $\sigma^\star$ regime in $\Sigma_{test}$?

\begin{figure}[!t]
  \raisebox{1.89cm}{
  \begin{minipage}{0.4\textwidth}
  \hspace{-0.5in}{\bf a.}\\
  \\
  \centering
  \begin{tikzpicture}
    \node[obs] (X) at (1.2, 0) {$X$};
    \node[fact] (F1) at (0.6, 1) {\textcolor{white}{$f_1$}};
    \node[fact] (F2) at (1.8, 1) {\textcolor{white}{$f_2$}};;
    \node[intv] (S1) at (0, 2) {$\sigma_1$};
    \node[intv] (S2) at (1.2, 2) {$\sigma_2$};
    \node[intv] (S3) at (2.4, 2) {$\sigma_3$};
    \edge[black]{S1}{F1};
    \edge[black]{S2}{F1};
    \edge[black]{S2}{F2};
    \edge[black]{S3}{F2};
    \uedge[black]{X}{F1};
    \uedge[black]{X}{F2};
  \end{tikzpicture}%
  \end{minipage}
  \begin{minipage}{0.4\textwidth}
  \hspace{-0.2in}{\bf b.}\\
  \\
  \begin{tikzpicture}
    \node[hobs] (F12) at (0, 3) {$(1, 2)$};
    \node[hintv] (FS2) at (1.2, 3) {$2$};
    \node[hobs] (F23) at (2.4, 3) {$(2, 3)$};
    \uedge[black]{F12}{FS2};
    \uedge[black]{FS2}{F23};
  \end{tikzpicture}%
  \end{minipage}
  \begin{minipage}{0.4\textwidth}
  \hspace{-0.2in}{\bf c.}\\
  \\
     \begin{tabular}{ccc}
     $\sigma_1$ & $\sigma_2$ & $\sigma_3$\\
     \hline
      0 & 0 & 0\\
      0 & 1 & 0\\
      1 & 0 & 0\\
      1 & 1 & 0\\
      0 & 0 & 1\\
      0 & 1 & 1\\
     \end{tabular}
 \end{minipage}}\\[-5mm]
 \vspace{-5mm}
 \caption{\textbf{(a)} An interventional factor graph with three intervention vertices. 
 \textbf{(b)} Intervention vertices can be arranged as a \emph{hypergraph} where hypervertex $(1, 2)$ represents set $(\sigma_1, \sigma_2)$ and an unboxed label represents the overlap between the two sets of intervention variables. 
 In \textbf{(c)}, a table showing the contents of a $\Sigma_{train}$ set. 
 From this set and the assumptions in \textbf{(a)}, it is possible to infer what happens when $\sigma_1 = \sigma_2 = \sigma_3 = 1$ (also true for the other missing entry, $\sigma_1 = \sigma_3 = 1$, $\sigma_2 = 0$). }
 \label{fig:identifiability_illustration}
 \vspace{-2mm}
\end{figure}

This identification problem is not analyzed in setups such as causal {B}ayesian optimization \citep{aglietti:20, sussex:23}, which model $p(x; \sigma)$ or $\mu(\sigma)$ directly. Without this analysis, it is unclear to what extent much of the learning is an artefact of the choice of prior distribution or regularization, particularly for a sparsely populated $\Sigma_{train}$. As an extreme case that is not uncommon in practice, if we have binary intervention variables and we never observe more than one $\sigma_i=1$ within the same experiment, it is unclear why we should expect a non-linear model to provide information about pairs of assignments $\sigma_i = \sigma_j = 1$ using an off-the-shelf prior or regularizer. Although eventually a dense enough process of exploration will enrich the database of experiments, this may be slow and less suitable to situations where the goal is not just to maximize some expected reward but to provide a more extensive picture of the dose-response relationships in a domain.

Furthermore, the smoothness of $p(x; \sigma)$ as a function of $\sigma$ may be relevant, it complicates identifiability criteria without further assumptions. In what follows, we will assume no smoothness conditions, meaning that for some pair $p(x; \sigma^a), p(x; \sigma^b)$, where $a \neq b$, such probability density/mass functions are allowed to be arbitrarily different. This is particularly important when interventions take categorical levels with limited to no magnitude information.

\paragraph{Identification: preliminaries.} 
Before introducing the main result of this section, let us start with a simple example from Figure~\ref{fig:identifiability_illustration}. 
The model in Figure~\ref{fig:identifiability_illustration}\textbf{(a)} shows a graph (how $X$ could be factorized is not relevant here), and Figure~\ref{fig:identifiability_illustration}\textbf{(c)} shows a set $\Sigma_{train}$ within a table. 
This set is lacking the experimental assignment $\sigma_1 = \sigma_2 = \sigma_3 = 1$.\footnote{As well as the assignment $\sigma_1 = \sigma_3 =  1, \sigma_2 = 0$, which can be recovered by an analogous argument.} 
However, this is implied by the graph and $\Sigma_{train}$. 
To see this, consider the implied factorization $p(x; \sigma) \propto f_1(x; \sigma_1, \sigma_2)f_2(x; \sigma_2, \sigma_3)$. 
This implies:
\[
\frac{p\big(x; (1, 1, 0)\big)}{p\big(x; (0, 1, 0)\big)} = \frac{f_1\big(x; (1, 1)\big)}{f_1\big(x; (0, 1)\big)},
\]
%\[
%\frac{p\big(x; (1, 1, 0)\big)}{p\big(x; (0, 1, 0)\big)} = \frac{f_1\big(x; (1, 1)\big)}{f_1\big(x; (0, 1)\big)} \frac{\cancel{f_2\big(x; (1, 0)\big)}}{\cancel{f_2\big(x; (1, 0)\big)}},
%\]
\noindent where we used $(1, 1, 0)$ etc. to represent assignments to $\sigma$ that should be clear from context. Because both $(1, 1, 0)$ and $(0, 1, 0)$ are in $\Sigma_{train}$, the ratio is trivially identifiable.

Moreover, multiplying and dividing the result by $f_2\big(x; (1, 1)\big)$, we get:
\[
\frac{p\big(x; (1, 1, 0)\big)}{p\big(x; (0, 1, 0)\big)} = \frac{f_1\big(x; (1, 1)\big)}{f_1\big(x; (0, 1)\big)}\frac{f_2\big(x; (1, 1)\big)}{f_2\big(x; (1, 1)\big)} = 
\frac{p\big(x; (1, 1, 1)\big)}{p\big(x; (0, 1, 1)\big)},
\]
\noindent from which, given that $(0, 1, 1)$ is also in $\Sigma_{train}$, we can derive $p\big(x; (1, 1, 1)\big)$.

The steps in this reasoning can be visualized in Figure~\ref{fig:identifiability_illustration}\textbf{(b)}. There, the leftmost \emph{hypervertex} represents $(\sigma_1, \sigma_2)$ and suggests $\sigma_1$ can be isolated from $\sigma_3$. The first ratio $p\big(x; (1, 1, 0)\big) / p\big(x; (0, 1, 0)\big)$ considers three roles: $\sigma_1$ can be isolated (it is set to a baseline of 1 in the denominator) and $\sigma_3$ is yet to be considered (it is set to a ``baseline'' value of 0 in the numerator). This ratio sets the stage for the next step, where $(\sigma_2, \sigma_3)$ is ``absorbed'' in the construction of the model evaluated at $(1, 1, 1)$. The entries in $\Sigma_{train}$ were chosen so that we see all four combinations of $(\sigma_1, \sigma_2)$, and all four combinations of $(\sigma_2, \sigma_3)$, while avoiding the requirement for all eight combinations of $(\sigma_1, \sigma_2, \sigma_3)$. 
How to generalize this idea is the challenge. Next, we present our proposed solution. 

\paragraph{Definitions.} Before we proceed, we need a few definitions. First, we call the regime $\sigma_1 = \sigma_2 = \dots = \sigma_d = 0$ the \emph{baseline} (or ``observational'') regime. This describes data captured under natural conditions with minimal effort, e.g. a transcriptomic study in which no genes are knocked down.

Let $\Sigma_{[S]}^0$ denote the set of all intervention levels $\sigma^i \in \Sigma$ such that $\sigma_j^i = 0$ iff $j \not \in S$. For instance, continuing the example in Figure~\ref{fig:graph_differences}\textbf{(b)}, a set $S := \{\sigma_2\}$ implies that $\Sigma_{[S]}^0 = \big\{(0, 0, 0), (0, 1, 0)\big\}$. 
%where $(0, 0, 0)$ is the assignment $\sigma_1 = \sigma_2 = \sigma_3 = 0$, and so on. 
%For some domain with $d = 4$ binary intervention variables $\{\sigma_1, \sigma_2, \sigma_3, \sigma_4\}$, the set $\Sigma_{[\{\sigma_1, \sigma_3\}]}^0$ is equal to $\{(0, 0, 0, 0), (1, 0, 0, 0), (0, 0, 1, 0), (1, 0, 1, 0)\}$.

An IFM $\mathcal I$ with intervention vertices $\sigma_1, \dots, \sigma_d$ has an associated \emph{$\sigma$-graph} denoted by $\mathcal G_{\sigma(\mathcal I)}$, and defined as an undirected graph with vertices $\sigma_1, \dots, \sigma_d$, and where edge $\sigma_i - \sigma_j$ is present iff $\sigma_i$ and $\sigma_j$ are simultaneously present in at least one common factor $f_k$ in $\mathcal I$. 

We also use the following concepts from graph theory as commonly applied to graphical models \citep{lauritzen:96, cowell:99}. 
% A \emph{decomposition} of an undirected graph $\mathcal G$ is formed from a partition of its vertices into a triplet $(A, B, C)$ where $C$ is complete (a clique) in $\mathcal G$ and separates $A$ from $B$. 
A \emph{decomposition} of an undirected graph $\mathcal G$ is formed from a partition of its vertices into a triplet $(A, B, C)$ where $C$ is complete  and separates $A$ from $B$. 
% A \emph{decomposition} of an undirected graph $\mathcal G$ is formed from a partition of its vertices into a triplet $(A, B, C)$, where $C$ is a complete subgraph/clique (with $|C|$ vertices) subgraph and separates $A$ from $B$ in $\mathcal G$. 
The decomposition is \emph{proper} if both $A$ and $B$ are non-empty. 
Moreover, an undirected graph is \emph{decomposable} if it is complete or, failing that, it has a proper decomposition into a triplet $(A, B, C)$, where the subgraph of $\mathcal G$ with vertices $A \cup B$ and the subgraph with vertices $B \cup C$ are both decomposable.

% Finally, a \emph{junction tree} $\mathcal T$ of a decomposable graph $\mathcal G$ is a tree where each vertex $V_i$ is labeled with the elements of a unique maximal clique from $\mathcal G$ (hence, this type of vertex is sometimes called a hypervertex), so that $V_i \cap V_j$ denotes the corresponding intersection among sets of vertices in $\mathcal G$. 
% Edges $V_i - V_j$ of $\mathcal T$ are graphically represented with labels denoting the intersection $V_i \cap V_j$. 
% A junction tree must have a \emph{running intersection} property: any intersection $V_i \cap V_j$ must be contained in all vertices in the (unique) path between $V_i$ and $V_j$ in $\mathcal T$.
Finally, a \emph{junction tree} $\mathcal T$ of a decomposable graph $\mathcal G$ is a maximum spanning tree $\mathcal T$, whose vertices corresponds to the maximal cliques of $\mathcal G$ and an edge between two such vertices, $V_i \text{ and } V_j$ in $\mathcal T$, corresponds to elements/variables that those maximal cliques share (i.e., $V_i \cap V_j$, with the edge weight given by the number of shared variables $|V_i \cap V_j|$). 
Thus, a junction tree has a \emph{running intersection} property: 
if two vertices $V_i$ and $V_j$ in $\mathcal T$ have variable(s) in common (i.e., $V_i \cap V_j \neq \emptyset$), then all vertices and edges in the (unique) path between $V_i$ and $V_j$ in $\mathcal T$ must also contain $V_i \cap V_j$.
% A junction tree must have a \emph{running intersection} property: any intersection $V_i \cap V_j$ must be contained in all vertices in the (unique) path between $V_i$ and $V_j$ in $\mathcal T$.

For instance, the $\sigma$-graph of the IFM represented in Figure~\ref{fig:identifiability_illustration}\textbf{(a)} is $\sigma_1 - \sigma_2 - \sigma_3$. 
This is a decomposable graph with vertex partition $A = \{\sigma_1\}$, $B = \{\sigma_2\}$ and $C = \{\sigma_3\}$. 
As this $\sigma$-graph is an undirected decomposable graph, it has a junction tree, which we depict in Figure~\ref{fig:identifiability_illustration}\textbf{(b)}, using boxes to highlight edge labels.

\paragraph{Identification: main result.} We are now ready to present the main result. Let $\mathcal I$ be an IFM representing a collection of probabilistic models for a random vector $X$ of dimension $m$ indexed by an intervention vector $\sigma$ of length $d$ and domain $\Sigma$. Model $\mathcal I$ has unknown factors but a known factorization $p(x; \sigma) \propto \prod_k f_k(x_{S_k}; \sigma_{F_k})$, where $S_k$ are subsets of $[m]$ and $F_k$ are subsets of $[d]$. Without loss of generality, we will assume no $F_k$ is contained in a different $F_{k'}$, so that maximal cliques in the $\mathcal G_{\sigma(\mathcal I)}$ have a one-to-one correspondence with sets $\{F_k\}$ (for instance, a factor $k$ which is not a function of any $\sigma$, i.e. $F_k = \emptyset$, can be absorbed by another factor for the following argument).

\begin{theorem}
 Assume that the $\sigma$-graph $\mathcal G_{\sigma(\mathcal I)}$ is decomposable. 
 Given a set $\Sigma_{train} = \{\sigma^1, \dots, \sigma^t\} \subseteq \Sigma$ and known distributions $p(x; \sigma^1), \dots, p(x; \sigma^t)$, the following conditions are sufficient to identify any $p(x; \sigma^\star)$, $\sigma^\star \in \Sigma$: 
 i) all distributions indexed by $\sigma^1, \dots, \sigma^t, \sigma^\star$ have the same support; and ii) $\Sigma_{[F_k]}^0 \in \Sigma_{train}$ for all $F_k$ in the factorization of $\mathcal I$.
\label{theorem:main}
\end{theorem}

(All proofs in Appendix \ref{appendix:proof}.) In particular, if no factor contains more than one intervention variable, the corresponding $\sigma$-graph will be fully disconnected. This happens, for example, for an IFM derived from a DAG without hidden variables and where each intervention has one child, as in Figure \ref{fig:graph_differences}. 

\begin{corollary}
Assume that the $\sigma$-graph $\mathcal G_{\sigma(\mathcal I)}$ is fully disconnected. Then any interventional distribution in $\mathcal I$ is identified by any $\Sigma_{train}$ where each level of each $\sigma_i$ appears along with baseline values for the other intervention variables.
\end{corollary}

It should be pointed out that a \emph{necessary} condition for identifiability is to have at least all combinations of values of $\sigma_{F_k}$ appearing in $\Sigma_{train}$. 
Whether it is possible to have a weaker sufficient condition than given by Theorem~\ref{theorem:main}, for instance not requiring a common baseline level in $\sigma_{\backslash F_k}$ at least once among each setting of $\sigma_{F_k}$, remains an open question.

\paragraph{Limitations of (non)decomposability.} If a $\sigma$-graph is not decomposable, the usual trick of triangulation prior to clique extraction can be used \citep{lauritzen:96,cowell:99}, at the cost of creating cliques which are larger than the original factors.
%In general, it is a price that needs to be paid. 
This cost is generally unavoidable.
For example, consider a variation of Figure~\ref{fig:identifiability_illustration}\textbf{(a)}, where a factor $f_3$ involving $\sigma_1$ and $\sigma_3$ is included. Following our construction, the corresponding $\sigma$-graph would be one big clique, and statements about $\sigma_1 = \sigma_2 = \sigma_3 = 1$ would not follow from Figure~\ref{fig:identifiability_illustration}\textbf{(c)}, \emph{even if} we were to add the regime $(1, 0, 1)$. 
%The following result formalizes this:
\begin{theorem}
Consider the IFM $p(x; \sigma) \propto f_1(x; \sigma_1, \sigma_2)f_2(x; \sigma_1, \sigma_3)f_3(x; \sigma_2, \sigma_3)$, where each $\sigma_i \in \{0, 1\}$. The distribution of this IFM under regime $\sigma_1 = \sigma_2 = \sigma_3 = 1$ cannot be identified from the other 7 possible regimes.
\end{theorem}

The main result shows that the factorization over $X$ is unimportant for identifiability, which may be surprising. We discuss the consequences of this finding to elicitation and testability in Appendix \ref{appendix:testability}.


==> macros.tex <==
\usetikzlibrary{cd,arrows,calc,shapes,positioning}
\tikzstyle{obs} = [circle,fill=white,draw=black,inner sep=0pt,minimum size=18pt,font=\fontsize{10}{10}\selectfont,node distance=1,thick]
\tikzstyle{latent} = [obs,dotted]

% Edge command from https://github.com/jluttine/tikz-bayesnet/blob/master/tikzlibrarybayesnet.code.tex
\newcommand{\edge}[3][]{ %
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={Latex[round]}, #1,thick] (\y) ;%
    } ;
  } ;
}

\definecolor{lightgrey}{rgb}{0.925, 0.925, 0.925}
\newcommand{\commentbox}[1]{\colorbox{lightgrey}{#1}}
\newcommand{\trueline}{\raisebox{2pt}{\tikz{\draw[black,solid,ultra thick](0, 0) -- (5mm, 0);}}}
\newcommand{\regressline}{\raisebox{2pt}{\tikz{\draw[black,dashed,ultra thick](0, 0) -- (5mm, 0);}}}
\newcommand{\boundline}{\raisebox{2pt}{\tikz{\draw[dotted,ultra thick](0, 0) -- (6mm, 0);}}}

\newcommand{\xhdr}[1]{\textbf{#1.}\;}

\newcommand{\bR}{\ensuremath \mathbb{R}}
\newcommand{\bN}{\ensuremath \mathbb{N}}
\newcommand{\cG}{\ensuremath \mathcal{G}}
\newcommand{\cB}{\ensuremath \mathcal{B}}
\newcommand{\cV}{\ensuremath \mathcal{V}}
\newcommand{\cE}{\ensuremath \mathcal{E}}
\newcommand{\cF}{\ensuremath \mathcal{F}}
\newcommand{\cJ}{\ensuremath \mathcal{J}}
\newcommand{\cL}{\ensuremath \mathcal{L}}
\newcommand{\cM}{\ensuremath \mathcal{M}}
\newcommand{\cS}{\ensuremath \mathcal{S}}
\newcommand{\cX}{\ensuremath \mathcal{X}}
\newcommand{\cY}{\ensuremath \mathcal{Y}}
\newcommand{\cZ}{\ensuremath \mathcal{Z}}
\newcommand{\cN}{\ensuremath \mathcal{N}}
\newcommand{\cD}{\ensuremath \mathcal{D}}
\newcommand{\pa}{\ensuremath \mathrm{pa}}
\newcommand{\cSconstr}{\ensuremath \overline{\mathcal{S}}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\E}{\mathbb{E}}
\DeclareMathOperator{\dist}{\mathrm{dist}}
\DeclareMathOperator{\indep}{\perp\!\!\!\perp}
\DeclareMathOperator{\dep}{\not\! \perp\!\!\!\perp}
\newcommand{\B}[1]{\bm{#1}}
\newcommand{\given}{\,|\,}
\newcommand{\lhslj}{\hat{\phi}_l(x_j, z_j)}
\newcommand{\lhs}{B}
\newcommand{\rhs}{A}
\newcommand{\obj}{\texttt{[obj]}}
\newcommand{\cdata}{\texttt{[c-data]}}
\newcommand{\cstruct}{\texttt{[c-struct]}}

